TSEmbed: Unlocking Task Scaling in Universal Multimodal Embeddings

Despite the exceptional reasoning capabilities of Multimodal Large Language Models (MLLMs), their adaptation into universal embedding models is significantly impeded by task conflict. To address this, we propose TSEmbed, a universal multimodal embedding framework that synergizes Mixture-of-Experts (MoE) with Low-Rank Adaptation (LoRA) to explicitly disentangle conflicting task objectives. Moreover, we introduce Expert-Aware Negative Sampling (EANS), a novel strategy that leverages expert routing distributions as an intrinsic proxy for semantic similarity. By dynamically prioritizing informative hard negatives that share expert activation patterns with the query, EANS effectively sharpens the model's discriminative power and refines embedding boundaries. To ensure training stability, we further devise a two-stage learning paradigm that solidifies expert specialization before optimizing representations via EANS. TSEmbed achieves state-of-the-art performance on both the Massive Multimodal Embedding Benchmark (MMEB) and real-world industrial production datasets, laying a foundation for task-level scaling in universal multimodal embeddings.

==> tables/Table_MMEB_dataset.tex <==
\begin{table}[!t]
\small
\centering
\caption{The statistics of MMEB: 36 datasets across 4 meta-task categories, with 20 in-distribution datasets used for training and 16 out-of-distribution datasets used exclusively for evaluation.}
\label{tab:mmeb_stat}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
  Meta-Task &
  Dataset &
  Query &
  Target &
  OOD? &
  \#Training &
  \#Eval &
  \#Candidates \\ \midrule
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}Classification \\ (10 Tasks)\end{tabular}} &
  ImageNet-1K &
  I &
  T &
   &
   100K
   &
  1000 &
  1000 \\ \cline{2-8} 
 & N24News           & I + T & I        &           &   49K & 1000 & 24   \\ \cline{2-8}  
 & HatefulMemes      & I        & T         &           &   8K & 1000 & 2    \\ \cline{2-8}  
 & VOC2007           & I        & T         &           &   8K & 1000 & 20   \\ \cline{2-8}  
 & SUN397            & I        & T         &           &   20K & 1000 & 397  \\ \cline{2-8}  
 & Place365          & I        & T         & \checkmark & - & 1000 & 365  \\ \cline{2-8}  
 & ImageNet-A        & I        & T         & \checkmark & - & 1000 & 1000 \\ \cline{2-8}  
 & ImageNet-R        & I        & T         & \checkmark & - & 1000 & 200  \\ \cline{2-8}  
 & ObjectNet         & I        & T         & \checkmark & - & 1000 & 313  \\ \cline{2-8}  
 & Country-211       & I        & T         & \checkmark & - & 1000 & 211  \\ \midrule
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}VQA \\ (10 Tasks)\end{tabular}} &
  OK-VQA &
  I + T &
  T &
   &
   9K
   &
  1000 &
  1000 \\ \cline{2-8} 
 & A-OKVQA           & I + T & T         &           &  17K & 1000 & 1000 \\ \cline{2-8}  
 & DocVQA            & I + T & T         &           &  40K & 1000 & 1000 \\ \cline{2-8}  
 & InfographicVQA    & I + T & T         &           &  24K & 1000 & 1000 \\ \cline{2-8}  
 & ChartQA           & I + T & T         &           &  28K & 1000 & 1000 \\ \cline{2-8} 
 & Visual7W          & I + T & T         &           &  70K & 1000 & 1000 \\ \cline{2-8}  
 & ScienceQA         & I + T & T         & \checkmark & - & 1000 & 1000 \\ \cline{2-8} 
 & VizWiz            & I + T & T         & \checkmark & - & 1000 & 1000 \\ \cline{2-8}
 & GQA               & I + T & T         & \checkmark & - & 1000 & 1000 \\ \cline{2-8}  
 & TextVQA           & I + T & T         & \checkmark & - & 1000 & 1000 \\ \midrule
\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Retrieval \\ (12 Tasks)\end{tabular}} &
  VisDial &
  T &
  I &
   &
  123K
   &
  1000 &
  1000 \\ \cline{2-8}  
 & CIRR              & I + T & I        &           &  26K & 1000 & 1000 \\ \cline{2-8}  
 & VisualNews\_t2i   & T         & I        &           &  100K & 1000 & 1000 \\ \cline{2-8}  
 & VisualNews\_i2t   & I        & T         &           &  100K & 1000 & 1000 \\ \cline{2-8}  
 & MSCOCO\_t2i       & T         & I        &           &  100K & 1000 & 1000 \\ \cline{2-8}  
 & MSCOCO\_i2t       & I        & T         &           &  113K & 1000 & 1000 \\ \cline{2-8}  
 & NIGHTS            & I        & I        &           &  16K & 1000 & 1000 \\ \cline{2-8}  
 & WebQA             & T         & I + T &           &  17K & 1000 & 1000 \\ \cline{2-8}  
 & OVEN              & I + T & I + T & \checkmark & - & 1000 & 1000 \\ \cline{2-8}  
 & FashionIQ         & I + T & I        & \checkmark & - & 1000 & 1000 \\ \cline{2-8}  
 & EDIS              & T         & I + T & \checkmark & - & 1000 & 1000 \\ \cline{2-8}  
 & Wiki-SS-NQ        & T         & I        & \checkmark & - & 1000 & 1000 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Visual Grounding\\ (4 Tasks)\end{tabular}} &
  MSCOCO &
  I + T &
  I &
   &
  100K
   &
  1000 &
  1000 \\ \cline{2-8} 
 & Visual7W-Pointing & I + T & I        & \checkmark & - & 1000 & 1000 \\ \cline{2-8}  
 & RefCOCO           & I + T & I        & \checkmark & - & 1000 & 1000 \\ \cline{2-8}  
 &
  RefCOCO-Matching &
  I + T &
  I + T &
  \checkmark &
  - &
  1000 &
  1000 \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/efficiency.tex <==
% Computational Efficiency Table
\begin{table}[t]
\centering
\caption{Computational efficiency comparison. We report training FLOPs, memory usage, and wall-clock time per epoch on MSCOCO with 8 V100 GPUs.}
\label{tab:efficiency}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Method} & \textbf{FLOPs} & \textbf{Parameters} & \textbf{Time/Step} & \textbf{Performance} \\
\midrule
Full Fine-tuning & 1.00× & 32.4 GB & 45 min & 70.3 \\
LoRA & 0.42× & 18.6 GB & 28 min & 72.6 \\
\textbf{\our} & 0.48× & 21.3 GB & 33 min & \textbf{77.2} \\
\midrule
Speedup vs. Full FT & 2.08× & 1.52× & 1.36× & +6.9 pts \\
\bottomrule
\end{tabular}%
}
\vspace{-0.1in}
\end{table}


